Counting Lyndon Subsequences

Counting substrings/subsequences that preserve some property (e.g., palindromes, squares) is an important mathematical interest in stringology. Recently, Glen et al. studied the number of Lyndon factors in a string. A string $w = uv$ is called a Lyndon word if it is the lexicographically smallest among all of its conjugates $vu$. In this paper, we consider a more general problem "counting Lyndon subsequences". We show (1) the maximum total number of Lyndon subsequences in a string, (2) the expected total number of Lyndon subsequences in a string, (3) the expected number of distinct Lyndon subsequences in a string.

==> macro.tex <==
\newcommand{\lcp}{\mathsf{lcp}}
\newcommand{\lynnum}{\mathit{L}}
\newcommand{\occ}{\mathit{Occ}}
\newcommand{\subcontain}{\mathit{C}}

\newcommand{\maxnum}{\mathit{MTS}}
\newcommand{\totalnum}{\mathit{TS}}
\newcommand{\distnum}{\mathit{MDS}}
\newcommand{\exnum}{\mathit{ETS}}
\newcommand{\totaldistinct}{\mathit{TDS}}
\newcommand{\exdistinct}{\mathit{EDS}}
\newcommand{\DF}{\mathit{MDF}}
\newcommand{\TF}{\mathit{MTF}}
\newcommand{\ETF}{\mathit{ETF}}
\newcommand{\EDF}{\mathit{EDF}}

